Medical AI Encodes a "Feeling of Error": Verifying Cancer Segmentation via Internal Concepts

Cancer segmentation models can fail silently, generating plausible but incorrect masks that risk missed findings or unnecessary biopsies. A critical question arises: Do AI models "know" when they are wrong, and if so, can we use the signal to predict their own failures? Humans do have a "Feeling of Error" (FOE): a spontaneous sense of unease that flags a potential error during thinking. We investigate whether cancer segmentation models exhibit an analogous internal signal. Unlike output-level cues (e.g., prediction confidence or uncertainty), which offer no insight into why a failure occurs and suffer from a sensitivity-quality tradeoff where high detection sensitivity could degrade overall segmentation quality. We instead propose to capture the model's FOE from its inner workings. Using mechanistic interpretability tools, specifically Sparse Autoencoders, we decompose internal neural activations into a dictionary of human-interpretable concepts and show that failure cases exhibit a distinct latent signature: fewer active concepts with lower activation magnitudes compared to successful segmentation. By training a classifier on these concept activations, we achieve accurate failure detection along with explanations for the model's mistakes. Experiments on prostate, pancreatic, and brain cancer segmentation demonstrate that our approach outperforms output-based methods in failure detection while preserving segmentation quality.

==> fig/concept_auroc.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{pic/concept_test_auroc.pdf}
  \caption{ ARUOC score for TP and FP masks on PI-CAI.}
  \label{fig:conceptauroc}
\end{figure}

==> fig/concept_pattern.tex <==
\begin{figure*}[thbp]
  % \dummyfig{TPs vs FPs concepts.}{0.30\linewidth}{0.98\textwidth}
  \includegraphics[width=\linewidth]{pic/tp_vs_fp_concept.pdf}
  \caption{Concept activation pattern for TP and FPs.}
  \label{fig:concept}
\end{figure*}

==> fig/fp_detection_brain.tex <==
\begin{figure}[t]
  \includegraphics[width=\linewidth]{pic/brain_fp_detection.pdf}
  \caption{F1 ($\uparrow$) vs. DSC ($\uparrow$) scores on MSD-Brain dataset. Each marker represents a baseline method varying by threshold [0.5, 0.8]. \textit{Our method surpasses the baseline Pareto front, achieving both higher DSC and higher F1, demonstrating superior reliability without sacrificing segmentation quality.}}
  \label{fig:brain}
\end{figure}

==> fig/title_figure.tex <==
\begin{figure}[t]
  % \dummyfig{Title figure}{0.45\linewidth}{0.45\textwidth} 
  \centering
  \includegraphics[width=0.5\linewidth]{pic/title.pdf}
  \caption{Comparison of failure detection approaches. Existing methods use uninterpretable output statistics from segmentation logits. Our approach extracts interpretable clinical concepts from internal representations, enabling failure interpretation via concept localization and failure correction.}
  \label{fig:title}
\end{figure}

==> tab/ablatin_layer.tex <==
% \begin{table}[!t]
% \centering
% \caption{Shallow vs. deep layer concepts for failure detection.}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lccc|c}
% % \toprule
% Layers (L)    & Early (L=1,3) & Mid (L=5,7) & Deep (L=9,11) & All \\ \midrule[1pt]
% DSC ($\uparrow$) &       &     &      &  50.1   \\
% F1 ($\uparrow$)  &       &     &      &   63.5  \\ 
% % \bottomrule
% \end{tabular}}
% \end{table}


% \begin{table}[!t]
% \centering
% \caption{Shallow vs. deep layer concepts for failure detection.}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lccc|c}
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Concept\\ Sources\end{tabular}} & Early       & Mid         & Deep         & \multirow{2}{*}{\textbf{All}} \\ \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} 
%                                                                            & Layers 1, 3 & Layers 5, 7 & Layers 9, 11 &                      \\ \midrule[1pt]
% DSC ($\uparrow$)                                                           &             &             &              & 50.1                 \\
% F1 ($\uparrow$)                                                            &             &             &              & 63.5                
% \end{tabular}}
% \end{table}

\begin{table}[!t]
\centering
\caption{Ablation on concept source layers. We compare performance when using concepts from only early, mid, or deep layers versus all layers combined. The full method (All) leverages complementary features to achieve the best performance.}
\resizebox{0.5\linewidth}{!}{%
\begin{tabular}{lccc|c}
\toprule
\multicolumn{1}{c}{Layers (L)} &  Early (1, 3) & Mid (5, 7) & Deep (9, 11)                 & All  \\ \midrule
DSC ($\uparrow$)                   &  47.5     &  48.8   & \multicolumn{1}{c|}{49.6} & \textbf{50.1} \\
F1 ($\uparrow$)                    &  44.5     &  50.4   & \multicolumn{1}{c|}{57.6} & \textbf{63.5} \\ \bottomrule
\end{tabular}}
\label{tab:layers}
\end{table}

==> tab/ablation_pooling.tex <==
\begin{table}[!t]
\centering
\caption{Aggregation methods.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|cccc}
% \toprule
Aggregation   & Mean & Max & Percentile (95\%) & L2 Norm\\ \midrule[1pt]
DSC ($\uparrow$) &  \textbf{50.1}     &     &   &   \\
F1 ($\uparrow$)  &  \textbf{63.5}     &     &   &  \\ 
% \bottomrule
\end{tabular}}
\end{table}

==> tab/ablation_sae.tex <==
% \begin{table}[!t]
% \centering
% \caption{Ablation on SAE architecture.}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{l|cccccc}
% % \toprule
% Dictionary Size (D)       & \multicolumn{3}{c}{D=1536 (768$\times$2)} & \multicolumn{3}{c}{D=768$\times$4=3072} \\ \cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
% Sparsity (S) & S=4    & S=8    & S=16   & S=4    & S=8    & S=16   \\ \midrule[1pt]
% DSC ($\uparrow$)      &    49.7    &   \textbf{50.1}     &  49.9      &        &        &        \\
% F1 ($\uparrow$)      &    60.3    &    \textbf{63.5}    &   62.5     &        &        &        \\ 
% % \bottomrule
% \end{tabular}}
% \label{tab:ablation_sae}
% \end{table}

\begin{table}[!t]
\centering
\caption{Ablation study on SAE architecture. We vary the dictionary size (D) and sparsity (S) and report the resulting failure detection F1 and segmentation DSC. The optimal configuration (D=1536, S=8) is in bold.}
\label{tab:sae_ablation}
\resizebox{0.5\columnwidth}{!}{%  <-- This scales the table to fit the column width
\begin{tabular}{l ccc ccc}
\toprule
 & \multicolumn{3}{c}{\text{D=1,536 (768$\times$2)}} & \multicolumn{3}{c}{\text{D=3,072 (768$\times$4)}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
\text{Sparsity (S)} & 4 & 8 & 16 & 4 & 8 & 16 \\
\midrule[1pt]
DSC ($\uparrow$) & 49.7 & \textbf{50.1} & 49.9 & 50.1 & 49.7 & 49.6 \\
F1 ($\uparrow$)  & 60.3 & \textbf{63.5} & 62.5 & 58.4 & 57.4 & 62.6 \\
% Average  & 55.0 & \textbf{56.8} & 56.2 & 54.3 & 53.6 & 56.1 \\
\bottomrule
\end{tabular}}
\label{tab:ablation_sae}
\end{table}

==> tab/albation_classifier.tex <==
\begin{table}[!t]
\centering
\caption{Ablation on the failure detection classifier. We compare performance using our SAE concepts with different classifiers. \textit{XGBoost achieves the best results for both DSC and F1.}}
\resizebox{0.5\linewidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Classifier    & XGB & Logistic & Decision Tree & Random Forest \\ \midrule[1pt]
DSC ($\uparrow$) &  \textbf{50.1}     &  47.8   &  48.5    &  44.6   \\
F1 ($\uparrow$)  &  \textbf{63.5}     &  59.2   &   58.7   &  57.0   \\ 
\bottomrule
\end{tabular}}
\label{ablation:classifier}
\end{table}

==> tab/feailure_detection.tex <==
% % \begin{table*}[h]
% % \centering
% % \resizebox{0.8\linewidth}{!}{%
% % \begin{tabular}{lcccccc}
% % \toprule
% % \multirow{2}{*}{} & \multicolumn{3}{c}{Prostate Cancer} & \multicolumn{3}{c}{Brain Cancer} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}
% %                   & FPR@95 ($\downarrow$)   &  DSC$^\star$ ($\uparrow$)  & F1$^\star$ ($\uparrow$)   & FPR@95 ($\downarrow$)   & DSC$^\star$ ($\uparrow$) & F1$^\star$ ($\uparrow$)  \\ \midrule
% % Threshold=0.5          &   /       &   51.9     & 35.9        &         &        &        \\
% % Threshold=0.6          &   /       &        & 35.9        &         &        &        \\
% % Threshold=0.7          &   /       &        & 35.9        &         &        &        \\
% % Threshold=0.8          &   /       &        & 35.9        &         &        &        \\
% % Threshold=0.9          &   /       &        & 56.4        &         &        &        \\ \midrule
% % Max Prob          &   53.3       &        &         &         &        &        \\
% % Mean Prob         &   52.4      &        &         &         &        &        \\
% % Entropy           &          &         &         &         &        &        \\ \midrule
% % Concept           &          &         &         &         &        &        \\
% % Raw embed.          &          &         &         &         &        &        \\ \midrule
% % Ours              &   \textbf{46.9}      &  \textbf{51.9}       &  \textbf{60.9}       &         &        &        \\ \bottomrule
% % \end{tabular}}
% % \caption{Failure detection accuracy.}
% % \end{table*}


% \begin{table*}[h]
% \centering
% \caption{FPR@95, DSC, and F1 scores on PI-CAI, BraTS, and MSD-Liver datasets.}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lccccccccc}
% \toprule
% \multirow{2}{*}{} & \multicolumn{3}{c}{PI-CAI (Prostate Cancer)} & \multicolumn{3}{c}{BraTS (Brain Cancer)} & \multicolumn{3}{c}{MSD-Liver (Liver Cancer)} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
%                   & FPR@95 ($\downarrow$)        & DSC ($\uparrow$)      & F1 ($\uparrow$)       & FPR@95 ($\downarrow$)        & DSC ($\uparrow$)      & F1 ($\uparrow$)      & FPR@95 ($\downarrow$)        & DSC ($\uparrow$)      & F1 ($\uparrow$)      \\ \midrule
% \multicolumn{10}{c}{\it Direct Thresholding}                                                                                                \\
% Threshold=0.5          &       /       &     \textbf{51.3}      &    35.9      &             &          &         &             &          &         \\
% Threshold=0.6          &      /        &    50.2       &  42.6        &             &          &         &             &          &         \\
% Threshold=0.7          &       /       &    46.8       &   49.3       &             &          &         &             &          &         \\
% Threshold=0.8          &      /        &    39.9       &   55.3       &             &          &         &             &          &         \\
% Threshold=0.9          &      /        &    19.1       &   \uline{56.4}       &             &          &         &             &          &         \\ \midrule
% \multicolumn{10}{c}{\it Output Logits or Confidence}                                                                                                \\
% MaxProb          &   53.3           &           &          &             &          &         &             &          &         \\
% MeanProb         &    52.4        &           &          &             &          &         &             &          &         \\
% Temp. Scaling           &              &           &          &             &          &         &             &          &         \\ 
% Entropy           &              &           &          &             &          &         &             &          &         \\ 
% Energy           &              &           &          &             &          &         &             &          &         \\ \midrule
% \multicolumn{10}{c}{\it Internal Representation}                                                                                                \\
% VLMs          &              &           &          &             &          &         &             &          &         \\
% % Ours (Raw embed.)           &   50.2           &           &  60.0        &             &          &         &             &          &         \\
% Ours (SAE$_\text{balance}$)             &     \textbf{xx.x}         &      xx.x     &    \textbf{xx.x}      &             &          &         &             &          &         \\
% Ours (SAE$_\text{aggressive}$)             &     \textbf{45.8}         &    xx.x       &    \textbf{63.5}      &             &          &         &             &          &         \\ \bottomrule
% \end{tabular}}
% \end{table*}

% \begin{table*}[ht]
% \centering
% \caption{FPR@95, DSC, and F1 scores on PI-CAI, BraTS, and MSD-Liver datasets.}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{llccccccccc}
% \hline
% \multicolumn{2}{l}{\multirow{2}{*}{}}                                                                   & \multicolumn{3}{c}{Prostate Cancer} & \multicolumn{3}{c}{Brain Cancer} & \multicolumn{3}{c}{Liver Cancer} \\ \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
% \multicolumn{2}{l}{}                                                                                    & FPR@95 $\downarrow$        & DSC $\uparrow$      & F1 $\uparrow$       & FPR@95 $\downarrow$        & DSC $\uparrow$      & F1 $\uparrow$      & FPR@95 $\downarrow$        & DSC $\uparrow$      & F1 $\uparrow$      \\ \midrule
% \multirow{10}{*}{\begin{tabular}[c]{@{}c@{}}\textit{\textbf{External}} \\ \textit{(Logits or}\\ \textit{Probability)}\end{tabular}} & Threshold=0.5       &   /           &    \textbf{51.3}       &   35.9       &             &          &         &             &          &         \\
%                                                                                        & Threshold=0.6      &     /         & 50.2          &  42.6        &             &          &         &             &          &         \\
%                                                                                        & Threshold=0.7      &     /         &    46.8       &  49.3        &             &          &         &             &          &         \\                                                                                       
%                                                                                        & Threshold=0.8 &      /        &   39.5        &     55.3     &             &          &         &             &          &         \\
%                                                                                        & Threshold=0.9        &   /           &     19.1      &   \uline{56.4}       &             &          &         &             &          &         \\ \cmidrule(lr){2-11}
%  & MaxProb       &   53.3           &     34.9      &    56.6      &             &          &         &             &          &         \\
%                                                                                        & MeanProb      &     52.4         &  29.9         &    53.0      &             &          &         &             &          &         \\
%                                                                                        & Temp. Scaling &              &           &          &             &          &         &             &          &         \\
%                                                                                        & Entropy &              &           &          &             &          &         &             &          &         \\
%                                                                                        & Energy        &              &           &          &             &          &         &             &          &         \\ \midrule
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textit{\textbf{Internal}} \\ \textit{(Concepts)}\end{tabular}}    & Ours (SAE$_\text{balance}$)        &              &           &          &             &          &         &             &          &         \\  
%                                                                                        & Ours (SAE$_\text{aggresive}$)           &      45.8        &   39.8        &   \textbf{63.6}       &             &          &         &             &          &         \\ 
% \end{tabular}}
% \end{table*}


% \begin{table*}[ht]
% \centering
% \caption{FPR@95, DSC, and F1 scores on PI-CAI, BraTS, and MSD-Liver datasets.}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{llccccccccc}
% \hline
% \multicolumn{2}{l}{\multirow{2}{*}{}}                                                                   & \multicolumn{3}{c}{Prostate Cancer} & \multicolumn{3}{c}{Brain Cancer} & \multicolumn{3}{c}{Liver Cancer} \\ \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
% \multicolumn{2}{l}{}                                                                                    & FPR@95 $\downarrow$        & DSC $\uparrow$      & F1 $\uparrow$       & FPR@95 $\downarrow$        & DSC $\uparrow$      & F1 $\uparrow$      & FPR@95 $\downarrow$        & DSC $\uparrow$      & F1 $\uparrow$      \\ \midrule
% \multirow{10}{*}{\begin{tabular}[c]{@{}c@{}}\textit{\textbf{External}} \\ \textit{(Logits or}\\ \textit{Probability)}\end{tabular}} & Threshold=0.5       &   /           &    \textbf{51.3}       &   35.9       &             &          &         &             &          &         \\
%                                                                                        & Threshold=0.6      &     /         & 50.2          &  42.6        &             &          &         &             &          &         \\
%                                                                                        & Threshold=0.7      &     /         &    46.8       &  49.3        &             &          &         &             &          &         \\                                                                                       
%                                                                                        & Threshold=0.8 &      /        &   39.5        &     55.3     &             &          &         &             &          &         \\
%                                                                                        & Threshold=0.9        &   /           &     19.1      &   {56.4}       &             &          &         &             &          &         \\ \cmidrule(lr){2-11}
%  & MaxProb       &   53.3           &     34.9      &    \uline{56.6}      &             &          &         &             &          &         \\
%                                                                                        & MeanProb      &     52.4         &  29.9         &    53.0      &             &          &         &             &          &         \\
%                                                                                        & Temp. Scaling &              &           &          &             &          &         &             &          &         \\
%                                                                                        & Entropy &              &           &          &             &          &         &             &          &         \\
%                                                                                        & Energy        &              &           &          &             &          &         &             &          &         \\ \midrule
% \multirow{1}{*}{\begin{tabular}[c]{@{}c@{}} \textit{\textbf{Internal}} \end{tabular}}    & Ours        &      \textbf{45.8}        &    50.1      &   \textbf{63.6}       &             &          &         &             &          &         \\  \bottomrule
% \end{tabular}}
% \end{table*}


\begin{table*}[!th]
\centering
\caption{FPR95 ($\downarrow$), AUROC ($\uparrow$), DSC ($\uparrow$), and F1 ($\uparrow$) scores on PI-CAI, PanTS, and MSD-Brain datasets.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{clcccccccccccc}
\toprule
\multicolumn{2}{l}{\multirow{2}{*}{}}                                                                   & \multicolumn{4}{c}{PI-CAI (Prostate Cancer)} & \multicolumn{4}{c}{PanTS (Pancreatic Cancer)} & \multicolumn{4}{c}{MSD-Brain (Brain Cancer)} \\ \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} 
\multicolumn{2}{l}{}                                                                                    & FPR95   & AUROC    & DSC    & F1   & FPR95   & AUROC   & DSC   & F1   & FPR95   & AUROC   & DSC   & F1   \\ \midrule
\multicolumn{14}{c}{\textit{Direct Thresholding on Probability Mask}} \\
\multirow{25}{*}{\begin{tabular}[c]{@{}c@{}}\\\textit{\textbf{External}}\\\textit{(logits or} \\ \textit{confidence)}\end{tabular}} & Threshold=0.5      &   /       &    /      &    \textbf{51.3}    &  35.9    &     /    &      /   &   31.1    & 22.0     &     /    &   /      & 66.0      & 84.7     \\
                                                                                       & Threshold=0.6      &   /       &    /      &   50.2     &  42.6    &   /      &     /    &    27.8   &   27.2   &     /    &       /  & 69.2      & 88.2     \\
                                                                                       & Threshold=0.7 &    /      &     /     &   46.8     &  49.3    &    /     &  /       &   18.2    &   35.4   &     /    &   /      & 70.9      & 89.2     \\
                                                                                       & Threshold=0.8        &     /     &    /      &   39.5     &   55.3   &   /      &     /    &    10.8   &  35.1    &   /      &     /    &   67.7    &   89.1   \\ \cmidrule(lr){2-14}
                                                                                       % & Threshold=0.9      &     /     &    /      &  19.1      &   56.4   &    /     &     /    &       &      &    /     &      /   &       &      \\ 
\multicolumn{14}{c}{\textit{Failure Detection Baselines with Threshold = 0.5}} \\
                                                                                       & MaxProb &   53.3       &   82.9       &   34.9     &  \uline{56.6}    &         &         &   7.53    &   21.9   & 17.9        & 94.7        &   62.7    & 90.2    \\
                                                                                       & MeanProb &     52.4     &    83.1      &    43.4    &  53.0    &         &         & 12.9      & 10.1     & 17.0       & 94.9        &    65.6   &   90.1   \\
                                                                                       & Entropy &    51.5      &    83.0      &   39.9     &  46.6    &         &         & 4.4      & 10.7     & 17.4        & 94.8        &   63.2    & 89.9     \\
                                                                                       & Energy        &  52.1        &   83.1       &  43.8      &  51.6    &         &         & 15.2      & 6.4     & 17.9        & 94.6        &   69.9    &  7.4    \\ \cmidrule(lr){2-14}
\multicolumn{14}{c}{\textit{Failure Detection Baselines with Threshold = 0.6}} \\
                                                                                       & MaxProb &   59.8      &  79.6        &    36.2   &  56.6    &         &         &   8.1    & 21.9     & 18,6        &  93.9       &    65.9   &  90.3    \\
                                                                                       & MeanProb &   55.0    & 80.0         &  41.3    &  50.8   &         &         &  9.3     &  1.0    & 17.6        & 94.1        &  68.3     & 90.0     \\
                                                                                       & Entropy &   56.3     &   80.0      &   40.1    &  51.7   &         &         &    9.5   &    25.3  & 18.4        & 93.9        & 66.7      & 90.2     \\
                                                                                       & Energy        &   54.7      &  80.1       &  41.5    &  49.5  &         &         &  11.5     &   0.0   & 18.7        & 93.9        & 68.4      & 0.0     \\ \cmidrule(lr){2-14}
\multicolumn{14}{c}{\textit{Failure Detection Baselines with Threshold = 0.7}} \\
                                                                                       & MaxProb &   65.3     &    78.6      &  36.7     &  56.6    &         &         &  0.0     &    0.0  & 22.7        & 92.4        &    68.5   &  90.3    \\
                                                                                       & MeanProb &   56.3    &   78.8       &   39.6   &  53.4   &         &         &  9.5     &  11.2    &  20.0       & 92.3        & 69.1      &   89.6   \\
                                                                                       & Entropy &    66.7    &  78.7       &  41.4     &  57.3   &         &         &   9.4    &  24.7    & 22.4        & 92.4        & 67.9      &  89.8    \\
                                                                                       & Energy        &    64.9     &   78.8      & 40.9     &  56.1  &         &         &    9.3   &    0.0  & 22.8       & 92.4        & 68.9     & 0.0    \\ \cmidrule(lr){2-14}
\multicolumn{14}{c}{\textit{Failure Detection Baselines with Threshold = 0.8}} \\
                                                                                       & MaxProb &    68.5     &  76.5        &   34.7   &  56.6    &         &         &   0.0    &   0.0   & 28.5        & 92.2        & 67.0      &   90.3   \\
                                                                                       & MeanProb &  72.6     &  76.6        &   36.0   & 54.9    &         &         &  0.0     &   0.0   & 27.7        & 92.1        & 67.2      &  90.3    \\
                                                                                       & Entropy &   70.1     &     75.8    &    36.4   & 56.4    &        &         & 10.1      & 1.1     &  27.7       & 92.2        & 66.6      &  90.1    \\
                                                                                       & Energy        &  70.2       &   75.8      &  28.0  &  36.2  &         &         &  0.0     &  0.0    & 28.5        &  92.2       &  64.5     &   0.0   \\ \cmidrule(lr){2-14}               
% \multicolumn{14}{c}{\textit{Failure Detection Baselines with Threshold = 0.9}} \\
%                                                                                        & MaxProb &  75.4       &    70.7      &  4.7     &    13.5  &         &         &       &      &         &         &       &      \\
%                                                                                        & MeanProb &  80.2     &  68.4        &   8.8   &   11.6  &         &         &       &      &         &         &       &      \\
%                                                                                        & Entropy &    79.7    &    68.5     &    9.5   & 14.3    &         &         &       &      &         &         &       &      \\
%                                                                                        & Energy        &    80.2     &   68.4      &  7.8    &  8.2  &         &         &       &      &         &         &       &      \\ \midrule
\textit{\textbf{Internal}}                                                                               & Ours           &   \textbf{45.8}       &     \textbf{85.7}     &   50.1    &  \textbf{63.5}    &         &         &       &      &         &         &   70.7    &  91.2   \\ \bottomrule
\end{tabular}}
\end{table*}

